Stepwise-Refining Speech Separation Network via Fine-Grained Encoding in High-order Latent Domain

The crux of single-channel speech separation is how to encode the mixture of signals into such a latent embedding space that the signals from different speakers can be precisely separated. Existing methods for speech separation either transform the speech signals into frequency domain to perform separation or seek to learn a separable embedding space by constructing a latent domain based on convolutional filters. While the latter type of methods learning an embedding space achieves substantial improvement for speech separation, we argue that the embedding space defined by only one latent domain does not suffice to provide a thoroughly separable encoding space for speech separation. In this paper, we propose the Stepwise-Refining Speech Separation Network (SRSSN), which follows a coarse-to-fine separation framework. It first learns a 1-order latent domain to define an encoding space and thereby performs a rough separation in the coarse phase. Then the proposed SRSSN learns a new latent domain along each basis function of the existing latent domain to obtain a high-order latent domain in the refining phase, which enables our model to perform a refining separation to achieve a more precise speech separation. We demonstrate the effectiveness of our SRSSN by conducting extensive experiments, including speech separation in a clean (noise-free) setting on WSJ0-2/3mix datasets as well as in noisy/reverberant settings on WHAM!/WHAMR! datasets. Furthermore, we also perform experiments of speech recognition on separated speech signals by our model to evaluate the performance of speech separation indirectly.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> tasnet.tex <==
The problem of single-channel speech separation can be formulated as: given a mixture of speech signal $\mathbf{x}\in \mathbb{R}^{1\times T}$ of temporal length $T$, the objective is to estimate the clean target sources $\mathbf{s_i}\in \mathbb{R}^{1\times T}, i=1,\dots,D$, where $D$ is the number of the involved speakers in the mixture. The time-domain audio separation network (TASNET)~\cite{TASNET}  performs separation through three stages: encoding, separating, and decoding, which are integrated into an end-to-end model. 

\subsection{Encoding}
\label{ssec:tasnet-enc}
The input speech signal is first divided into $T'$ overlapped segments of length $K$, and then each segment is transformed into a $N$-dimensional vector. The obtained vectors are concatenated into a 2-D representation $\mathbf{F} \in \mathbb{R}^{N\times T'}$. Formally, the encoder $\mathcal{E}$ encodes the input mixture $x$ into an embedding space with $N$ basis functions:
\begin{equation}
\mathbf{F} = \mathcal{E} (\mathbf{x}).
\end{equation}
Specifically, the encoder is modeled by a 1-D convolutional layer with $N$ filters of kernel size $K$ followed with the nonlinear activation layer. Herein, the $N$ convolutional filters can be viewed as the basis functions to form a latent domain, which presumably simulates the frequency domain due to the similar mathematical transformations between the CNN encoder and the Short-Time Fourier Transformation~\cite{STFT}. 

\subsection{Separating}
\label{ssec:tasnet-sep}

The encoded representation $\mathbf{F}$ is fed into the separator $\mathcal{S}$ to estimate the mask $\mathbf{M_i} \in \mathbb{R}^{N\times T'}, i=1,\dots,D$ for each source, thus the separated representation $\mathbf{F_i} \in \mathbb{R}^{N\times T'}, i=1,\dots,D$ is obtained by applying the corresponding mask to the encoded mixture representation $\mathbf{F}$: 
\begin{equation}
\begin{split}
    & \mathbf{M_i} = \mathcal{S} (\mathbf{F}) \\
    & \mathbf{F_i} = \mathbf{M_i} \odot \mathbf{F},
\end{split}
\end{equation}
where $\odot$ denotes element-wise multiplication.
The crux of representation separation is how to perform effective temporal modeling for the extremely long encoded sequential representation. Variants of TASNET are proposed to solve this problem through devising efficient separator, including Conv-TASNET~\cite{Conv-tasnet}, FurcaNeXt~\cite{furcanext}, DPRNN-TASNET~\cite{DPRNN}, SuDoRM-RF~\cite{sudo}, DPTNET-TASNET~\cite{DPTNet}, and SepFormer~\cite{SepFormer}, while DPRNN-TASNET and DPTNET-TASNET are two performant and lightweight variants among them.

%In Conv-TASNET~\cite{Conv-tasnet}, the fully-convolutional separator consists of stacking 1-D dilated temporal convolutional blcoks~\cite{TCN, dilated}. $M$ stacking convolutional dilated blocks with dilation rates of $2^0, 2^1, \dots, 2^{M-1}$ are repeating $R$ times. The exponentially increasing dilation rates allow the convolutional layers to model large temporal context without increasing parameters proportionally ~\cite{TCN}. With each convolutional block, standard convolutional layer is replaced with depthwise separable convolutional layer \cite{mobilenets,xception}, which further decreases the model size. On the top of the convolutional blocks, a 1-D convolutional layer with kernel size of 1 is utilized to estimate the masks. 

Dual-Path RNN (DPRNN)~\cite{DPRNN} is developed to capture long-time dependency which models the entire sequential inputs instead of fixed receptive fields in Conv-TASNET~\cite{Conv-tasnet}. It consists of three steps: segmentation, temporal modeling, and overlap-add operation. Firstly, the sequential representation is segmented into overlapping chunks. Then $R$ stacking blocks of DPRNN are utilized for for long-time modeling. Each block is composed of two RNN layers: intra-RNN and inter-RNN. The intra-RNN is applied within each chunk independently, which models local temporal information. The inter-RNN is applied across different chunks, which models the global temporal information. Thirdly, after time-domain modeling, the overlapping chunks are transformed back into sequential shape through the overlap-add operation~\cite{DPRNN}. 

Dual-Path Transformer Network (DPTNet)\cite{DPTNet} also adopts the dual-path strategy to handle the long sequence through three steps: segmentation, temporal modeling, and overlap-add operation. $R$ stacking blocks of DPTNet are utilized for for long-time modeling. Similar to DPRNN~\cite{DPRNN}, each block of DPTNet consists of two order-aware transformer layers: intra-transformer and inter-transformer, which model local (intra-chunk) and global (inter-chunk) temporal information in an alternate manner. In order to learn order information, the first fully connected layer in the feed-forward network of the standard transformer layer~\cite{transformer} is replaced with an RNN layer. With the self-attention computation in transformer layer, different time steps can interact directly without intermediate transmission as in RNN layers~\cite{self-acoustic}. 

\subsection{Decoding}
\label{ssec:tasnet-dec}

After obtaining the separated representations $\mathbf{F_i}$ in the encoding space, the decoder $\mathcal{D}$ reconstructs the speech sources $\mathbf{s}_i \in \mathbb{R}^{1\times T}, i= 1, \dots, D$ for each speaker:
\begin{equation}
    \mathbf{s}_i = \mathcal{D} (\mathbf{F}_i), i = 1, \dots, D.
\end{equation}
The decoder $\mathcal{D}$ is modeled as a 1-D transposed convolutional layer which is the reversed operation of the encoder $\mathcal{E}$.









